FASHION: Functional and Attack graph Secured HybrId Optimization of virtualized Networks

Maintaining a resilient computer network is a delicate task with conflicting priorities. Flows should be served while controlling risk due to attackers. Upon publication of a vulnerability, administrators scramble to manually mitigate risk while waiting for a patch. We introduce FASHION: a linear optimizer that balances routing flows with the security risk posed by these flows. FASHION formalizes routing as a multi-commodity flow problem with side constraints. FASHION formulates security using two approximations of risk in a probabilistic attack graph (Frigault et al., Network Security Metrics 2017). FASHION's output is a set of software-defined networking rules consumable by Frenetic (Foster et al., ICFP 2011). We introduce a topology generation tool that creates data center network instances including flows and vulnerabilities. FASHION is executed on instances of up to 600 devices, thousands of flows, and million edge attack graphs. Solve time averages 30 minutes on the largest instances (seconds on the smallest instances). To ensure the security objective is accurate, the output solution is assessed using risk as defined by Frigault et al. FASHION allows enterprises to reconfigure their network in response to changes in functionality or security requirements.

==> appendex.tex <==
%!TEX root = main.tex
\section{Appendix}


\subsection{Approximation bounds}
For the purpose of finding the bounds on our approximation, we will consider the static formulation for $risk$. 

\begin{lemma}
  \label{no zeroes}
  For any $v\in V(G)$ such that $0 = P(v)$, removing all $\delta^+(v)$ and $\delta^-(v)$ from $E(G)$ will have no effect on $risk(G)$.
\end{lemma}
\begin{proof}
\end{proof}
\begin{remark}
  Any zero probability in $P$ is equivalent to having a partially disconnected graph.
\end{remark}

\begin{lemma}
  \label{edge removal}
  Let $G$ be some DAG such that $G$ is not complete. Than adding another edge to $G$ will monotonically increase $risk(G)$
\end{lemma}
\begin{proof}
  Let $G$ be a graph as described above. Than we can add some edge, $e=(i, j)$, to $G$ in a place where no edge exists, in a direction such that no cycle is created. Because we've added a new edge, we've increased the size of $\delta^-(v)$ for some $v\in V$. Thus, some number of $L(v)$ must increase (or remain fixed), without any restrictions on $C(V)$. Because of this, $risk(G)$ also increases.
\end{proof}
Thus, if our goal is to minimize $risk(G)$, we need to minimize $|E(G)|$. In order to go about this, we can attempt to remove the $k_3$ minors from the graph.

\begin{lemma}
  \label{vertex removal}
  Adding a vertex to $G$ while keeping $G$ connected will always increase $risk$ 
\end{lemma}
\begin{proof}
\end{proof}
\begin{remark}
  While removing all vertices from a graph or disconnecting the graph (these are equivalent for minimizing risk) does minimize risk, it also makes the problem less interesting overall. Thus we will be considering only cases for which the graph is connected, including the requirements of \autoref{no zeroes}.
\end{remark}

\begin{theorem}
  A path graph ($P_n$) is minimal in terms of risk for a connected graph.
\end{theorem}
\begin{proof}
  Consider a graph that is not a path graph. Let $G$ be an arbitrary graph. By \autoref{edge removal} we know that any $k_3$ minor in $G$ will result in an unnecessary increase in $risk(G)$. For each $k_3$ minor in $G$, we remove an edge such that no $L(v) = 0$ for all $ v\in V(G)$. since $G$ is now minimally connected it must be a rooted \todo{arborescence vs polytree?}{polytree}.
  We show by induction on the number of leaves of $G$, that a chain graph is less than or equal in $risk$ to the original graph structure. In the base case where the number of leaves is $1$, the graph is a chain, and the risk is 
  $$
    risk(G) = \sum_{{v_n\in V(G)}}\prod_{{i=0}}^{n}p_i
  $$
  Now consider a graph of $n$ nodes and $k$ leaves. Since the number of leaves is not 1, there must exist at least 2 branches, $B_1$ and $B_2$, such that the branching factors are both 1 (both sub-graphs are chains), and for which $B_1$ and $B_2$ have the same fork as an endpoint (both start at the same vertex). Since these branches are themselves chain graphs, we can compare their contributions to $risk(G)$ by treating the fork as the root of the tree.  Without loss of generality, we consider the case of $risk(B_1)\leq risk(B_2)$. We can reconstruct the tree such that $B_2$ directly follows the leaf vertex of $B_1$. This operation is non-increasing.
\end{proof}
\begin{remark}
   The path graph has a risk formulation of $$risk(G)=\sum_{\mathclap{i=1}}^{\mathclap{|V(G)|}}p^i\times C(V(G)_i)$$ where $p$ is the probability of reaching a vertex on the graph. If we fix $C(v)$ to be a constant $c$, than $$risk(G)=\frac{pc\left(1-p^{|V(G)|}\right)}{1-p}$$
\end{remark}

Re-add in positions such that (comparator for sorting), where $p_2$ is being added before $p_1$
$$
\frac{p_1 c_1}{1-p_1} \geq \frac{p_2 c_2}{1-p_2}
$$
to ensure
$$
p_1 c_1 + p_1 p_2 c_2 \leq p_2 c_2 + p_1 p_2 c_1
$$

\begin{corollary}
  Since a path graph is minimal in terms of risk, the approximation is bounded by
  $$O(v,p) = \lim_{\mathclap{v,p\to\infty}}\;\frac{v(1-1/p)}{(1-(1/p)^v)/p}=\frac{vp-v}{1-(1/p)^v}= vp-v=vp$$
\end{corollary}

\subsection{Additional Clusters}
\begin{figure}[htp]
\centering
\includegraphics[width=0.5\textwidth]{figures/heuristics/riskpod6cluster1.pdf}
\caption{Cluster 1}
\label{fig:cluster1}
\end{figure}

\begin{figure}[htp]
\centering
\includegraphics[width=0.5\textwidth]{figures/heuristics/riskpod6cluster3.pdf}
\caption{Cluster 3}
\label{fig:cluster3}
\end{figure}

\begin{figure}[htp]
\centering
\includegraphics[width=0.5\textwidth]{figures/heuristics/riskpod6cluster5.pdf}
\caption{Cluster 5}
\label{fig:cluster5}
\end{figure}

\begin{figure}[htp]
\centering
\includegraphics[width=0.5\textwidth]{figures/heuristics/riskpod6cluster7.pdf}
\caption{Cluster 7}
\label{fig:cluster7}
\end{figure}

==> old_stuff.tex <==
\appendix
\section{Old Stuff maybe to use}
\input{approximation}
\subsection{ Probabilistic Risk Analysis}
\begin{itemize} \item
We implement a probabilistic Risk Analysis as is found in previous work by Wang \textit{et al.} \cite{Wang2008}.  
\cite{Frigault2008a}
Frigault et al. utilizes  Bayesian Networks as model to generate their attack graphs in measuring network security which has been criticized for their limited ability to deal with cycles.

\item \cite{Homer2009,Homer2013}
Homer et al. present a provably sound quantative model to predect the likleyhood of a network breach in an enterprise network.  Provides a strong argument for the requirement for clear metric semantics regarding  Network Risk and Attack Graphs.  Similar to Frigault et al. \cite{Frigault2008a} states that Bayesian Networks are good finding cumulative probability but have difficulty correctly evaluating cycles due to a self-referencing effect.  They also provide that methods for dealing with cycles such as unfolding present the additional complexity and may result in intractability.

\end{itemize}
\subsection{Old stuff}
\ben{to use?}

A major advantage to our implementation of Attack Graphs over existing work is the real-time integration of the Network  reachability decisions and the associated risk theses decisions create. Historically Attack Graphs have been generated from a static network configuration without the ability for interplay with network reachability but rather a static risk assessment. In our implementation combining Optimization with SDN, network reachability information is centrally available and configurable without requiring reachability scanns.
We leverage the notion that each vulnerability has a probability of being exploited, which is reflected in the exploitability score found in CVSS. 

 In the spirit of the NIST cybersecurity framework \cite{website:CF} we include an importance metric for each
network resource,this approach allows customization of resource criticality based on
unique business practices or mission constraints.  We establish a reachability model that
includes network resources combined with access privilege level. Privilege is
defined through a combination of ownership (user, group, other) and file privilege (read, write and execute) are standard across UNIX operating systems \cite{Stevens2008}.  

Each network resource is assigned a criticality and combined with its propensity for
unwanted reachabiltiy we derive a security score for the network configuration.  Note that this security score is relative to other similar configurations (hosts, vulnerabilities, importance metrics) and not as a quantitative stand-alone metric.  

In establishing our Attacker model we assume a strong adversary with respect his ability to conduct successfull exploits.  This is similar the process used in \cite{Ingols2006} and also widely used by the United States Military in their Operation Planning approach of determining the enemies most dangerous course of action \todo{ATP 2-01.3}. This approach is taken for two reasons, 1. We insure that we dont underestimate the threat to the network which could be the case in a true probabalistic/Bayesian approach \cite{Homer2013} . 2. A benefit to our worst-case approach is seen in the speed to generate the Attack Graph when compared general Bayesian Network Attack Graphs.(give speedup )  This speedup allows us to overcome the timing barriers that historically prevent Attack Graphs from being useful in a real-time system.  To ensure flexibility we provide a threshold which allows us to convert all probabilities into a boolean and then generate the Attack Graph deterministically.

A typical limitation to Attack Graph utilization is the combinatorial growth relative to the number of hosts which makes them too large/slow to compute for networks of scale\cite{Ingols2006}.  This problem is overcome by the white list routing approach of our network.  In typical networks there is often an all
to all routing approach where each host is capable of reaching each host.  This is
contrary to our approach where we only provide reachabiltity between allowable hosts or
processes.   \

